Keeping Notes: Conditional Natural Language Generation with a Scratchpad Mechanism

We introduce the Scratchpad Mechanism, a novel addition to the sequence-to-sequence (seq2seq) neural network architecture and demonstrate its effectiveness in improving the overall fluency of seq2seq models for natural language generation tasks. By enabling the decoder at each time step to write to all of the encoder output layers, Scratchpad can employ the encoder as a "scratchpad" memory to keep track of what has been generated so far and thereby guide future generation. We evaluate Scratchpad in the context of three well-studied natural language generation tasks --- Machine Translation, Question Generation, and Text Summarization --- and obtain state-of-the-art or comparable performance on standard datasets for each task. Qualitative assessments in the form of human judgements (question generation), attention visualization (MT), and sample output (summarization) provide further evidence of the ability of Scratchpad to generate fluent and expressive output.

==> figs/baselines.tex <==
\begin{table}[h]
\makebox[\textwidth][c]{
{\renewcommand{\arraystretch}{1.25}
\begin{tabular}{l c c c c c c}
\toprule
Name & \makecell{Replace \\ Entity ID} & \makecell{Glove Word \\ Embeddings} & Beam Search & Ability to Copy & \makecell{Coverage \\ RNN} & \makecell{Scratchpad \\ Encoder} \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}


Seq2Seq & \xmark & \xmark & \xmark & \xmark & \xmark  & \xmark \\ 
+ Priors & \cmark & \cmark & Beam Size 2& \xmark & \xmark  & \xmark \\ 

\cmidrule(lr){1-7}

Copynet & \cmark & \cmark & \xmark & \cmark & \xmark & \xmark \\
+ Coverage & \cmark & \cmark & \xmark & \cmark & \cmark & \xmark\\
+ Scratchpad & \cmark & \cmark & \xmark & \cmark & \xmark & \cmark \\

\bottomrule
\end{tabular}}
}
\caption{To validate the method, we compare against a pure \textit{seq2seq with attention} baseline, along with a tuned (``+ Priors") version and a \textit{Copynet} with the same improvements except for beam search. We then enhance a copynet with a \textit{coverage mechanism} and a \textit{scratchpad encoder}.}
\label{table:baselines}
\end{table}

==> figs/copy_misfires.tex <==
\begin{table}[h]
\begin{tabularx}{\linewidth}{Y Y Y Y}
\toprule
Expected & Copynet & Coverage & Scratchpad \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
what was thomas jefferson role in the declaration of independence?
& what is jefferson \textbf{\textcolor{red}{jefferson}} famous for?
& what was thomas jefferson famous for?
& what jobs did thomas jefferson have?\\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
who does chris hemsworth have a baby with?
& what does chris \textbf{\textcolor{red}{chris chris}} with?
& who is chris \textbf{\textcolor{red}{chris}} hemsworth?
& who is chris hemsworth married to?\\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
what type of music did vivaldi compose?
& what type of music did vivaldi \textbf{\textcolor{red}{vivaldi}} sing?
& what music did antonio vivaldi compose?
& what music did antonio vivaldi compose?\\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
what else did ben franklin invent?
& what is the inventions \textbf{\textcolor{red}{inventions}} of franklin \textbf{\textcolor{red}{franklin}}?
& what was the inventions benjamin \textbf{\textcolor{red}{benjamin}} franklin's children?
& what are some inventions benjamin franklin made?\\

\bottomrule
 \end{tabularx}
\caption{Example instances from the test set of the copy-mechanism of \textit{copynet} over-firing where the \textit{scratchpad} model copies correctly.}
\label{table:copy_misfires}
\end{table}

==> figs/copyable_tokens.tex <==
\begin{table}[!htbp]
\centering
\framebox(320, 70){
\makebox[\textwidth][c]{
\begin{tabular}{l}
%\hline
what are the \textbf{official} languages in \textbf{spain} ?\\ %\hline
%what \textbf{country} is the \textbf{grand bahama} island in ?\\ %\hline
what is the first \textbf{book sherlock holmes appeared} in ?\\ %\hline
when did the \textbf{new york knicks} win a \textbf{championship} ?\\ %\hline
who portrayed \textbf{indiana jones} in \textbf{raiders of the lost ark} ?\\ %\hline
from what \textbf{university} did \textbf{president obama} receive his \textbf{bachelor} 's \textbf{degree} \\ %\hline
\end{tabular}
}}
%\parbox{0.75\textwidth}{
\captionsetup{width=.9\linewidth}
\centering
\caption{Example questions from the training set of WebQuestionsSP dataset, with tokens that also appear in the sparql in bold. Nearly half ($47.36\%$) of tokens in questions appear in the corresponding sparql, suggesting that the ability to copy can improve performance on this task.}
%}
\label{table:copyable_tokens}
\end{table}

==> figs/prepro.tex <==
\begin{figure}[t]
\framebox(395, 175){
\makebox[\textwidth][c]{
\begin{tabular}{l}

%\shortstack[l]{
{\fontsize{7}{9 }\selectfont \makecell[l]{
 %\\
 SELECT DISTINCT ?x \\
 WHERE \{ \\
 FILTER (?x != ns:m.01bkb) \\
 FILTER (!isLiteral(?x) OR lang(?x) = '' OR langMatches(lang(?x), 'en')) \\
 ns:m.01bkb ns:travel.travel\_destination.how\_to\_get\_here ?y .\\
 ?y ns:travel.transportation.transport\_terminus ?x .\\
 ?y ns:travel.transportation.mode\_of\_transportation ns:m.03qb78c . \\
\}
} }\\ 
\multicolumn{1}{c}{\fontsize{9}{11}\selectfont (Raw)} \\
\cmidrule(lr){1-1}
{\fontsize{7}{9 }\selectfont \makecell[l]{
 %\\
 select distinct ? x \\
 where \{ \\
 filter ( ? x ! = ent: bali ) \\
 filter ( ! is literal ( ? x ) or lang ( ? x ) = ' ' or lang matches ( lang ( ? x ) , ' en ' ) ) \\
 ent: bali ns travel . travel \_ destination . how \_ to \_ get \_ here ? y . \\
 ? y ns travel . transportation . transport \_ terminus ? x .
 ? y ns travel . transportation . mode \_ of \_ transportation ent: air transportation . \\
 \} 
}} \\
\multicolumn{1}{c}{\fontsize{9}{11}\selectfont (Preprocessed)} \\
\end{tabular}
}}
\caption{To preprocess SPARQL, we split on: special characters ($? \ ! \ = \ : \ . \ \un \ ( \ ) \ \{ \ \} \ '$), ':' not followed by '/', and camelCasing. Entity IDs are replaced with the 'ent:' token followed by the entity's full name. We then lowercase all strings. }
\label{fig:prepro}
\end{figure}

==> figs/seq_sql_misfires.tex <==
\begin{table}[h]
\begin{tabularx}{\linewidth}{Y Y Y Y}
\toprule
Expected & Copynet & Coverage & Scratchpad \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
what is the total number of attendance ( s ) , when away is real juventud ?
& what was the attendance for juventud \textbf{\textcolor{red}{juventud}} ?
& what was the attendance against real juventud ?
& what was the total attendance against real juventud \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
name the pictorials when the interview subject is steve jobs
& in the issue in which the steve were \textbf{\textcolor{red}{were}} steve \textbf{\textcolor{red}{steve}} , what were the steve ?
& in the issue in \textbf{\textcolor{red}{in in}} the issue where jobs \textbf{\textcolor{red}{jobs}} was the interview subject
& which were the pictorials in which the interview subject was steve jobs ?\\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
name the \% of popular vote for election for 1926
& what is the percentage of the vote 1926 in \textbf{\textcolor{red}{1926}} ?
& what is the percentage of the vote in the candidate of 1926 ?
& what was the percentage of popular vote for the 1926 election ?\\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
what is the lowest rank ?
& what is the smallest rank ? a \textbf{\textcolor{red}{rank ?}}
& what is the smallest rank for a \textbf{\textcolor{red}{rank}} ?
& what 's the minimal rank of a athlete shown in the chart ?\\

\bottomrule
 \end{tabularx}
\caption{Example instances from the test set of the copy-mechanism of \textit{copynet} over-firing where the \textit{scratchpad} model copies correctly.}
\label{table:copy_misfires}
\end{table}

==> figs/summarization_examples.tex <==
% defining our colours to be used in figures
\definecolor{gred}{RGB}{219,68,55}
\definecolor{gblue}{RGB}{66,133,244}
\definecolor{gyellow}{RGB}{244,180,0}
\definecolor{ggreen}{RGB}{15,157,88}
\definecolor{ggrey}{RGB}{115,115,115}
\newcommand{\hlpgen}[2]{\fboxsep1pt \colorbox{ggreen!#2}{\strut #1}} % highlight text with custom saturation. for pgen
\newcommand{\hlcov}[2]{\fboxsep1pt \colorbox{gyellow!#2}{\strut #1}} % highlight text with custom saturation. for cov
\newcommand{\error}[1]{\textcolor{gred}{\textbf{#1}}} % highlight errors in examples
\newcommand{\fph}[1]{\textcolor{gblue}{\textbf{#1}}} % highlight source of final summary in first page example
\newcommand{\reph}[1]{\textcolor{ggreen}{\textbf{#1}}} % highlight repetition in first page example
\newcommand{\novelh}[1]{\textcolor{gblue}{\textbf{#1}}} % highlight novel words in the figure of abstractive examples

\begin{figure}[H]
\begin{boxedminipage}{\columnwidth}
\scriptsize
% \footnotesize
% \small
\textbf{Original Text (truncated):}
In a quest to be more green , Apple says it is investing in Chinese solar power and preserving American forests that make environmentally friendly paper . The tech giant announced a new focus on using paper from trees harvested under environmentally sound conditions . As part of the deal , Apple has pledged an unspecified amount of money for a Virginia-based nonprofit , the Conservation Fund , to purchase two large tracts of timberland on the East Coast . Then EPA Administrator Lisa Jackson , now Apple 's president for environmental initiatives , has spearheaded the new green focus at the world 's biggest company . Apple pledged an unspecified amount of money for a Virginia-based nonprofit , the Conservation Fund , to purchase two large tracts of timberland on the East Coast . ...
%In the Reed Forest of Aroostook County , Maine , wetlands , rivers , and upland forest provide refuge for Atlantic salmon , bald eagle , and Canada lynx . In Brunswick Forest located in southern North Carolina , the high-quality pine savannas and unique plants and flowers have long made this land a conservation priority . The Conservation Fund will resell the land to commercial interests under legally binding terms that require future owners to preserve the forest and follow environmentally sound principles for cutting and replanting trees . The initiatives come as the tech giant this year met a self-imposed goal of powering all its U.S. operations with renewable energy to reduce carbon emissions -- initiatives that have won high marks from environmental groups . On Thursday , It 's also promising to use more renewable power overseas , where Apple relies heavily on contract manufacturers -- and where a top executive acknowledged the company can do more . `` It 's important to us to tackle climate change everywhere we are , '' Lisa Jackson , Apple 's vice president for environmental initiatives , told The Associated Press . `` When you talk about China , you 're talking about manufacturing partners . '' `` We 're looking to bring the same innovation there . '' `` This is the start . '' The new solar project in China has a capacity of 40 megawatts , which is smaller than some projects Apple has announced in the United States . By comparison , Apple is spending \$ 850 million for rights to nearly half the output of a 280-megawatt solar facility planned for construction south of Apple 's Cupertino , California , headquarters . That project will produce enough energy to power all of Apple 's California offices , a computer center and 52 retail stores .
\newline \rule{\columnwidth}{1.2pt}
\textbf{Reference:}
apple helping nonprofit buy large tracts of timberland on the east coast. 
firm now powers u.s. operations with renewable energy. 
\newline \rule{\columnwidth}{0.4pt}
\textbf{Scratchpad:}
the tech giant announced a new focus on using paper from trees harvested under environmentally sound conditions.
as part of the deal , apple has pledged an unspecified amount of money for a virginia-based nonprofit , the conservation fund , to purchase two large tracts of timberland on the east coast.
then epa administrator lisa jackson , now apple 's president for environmental initiatives , has spearheaded the new green focus at the world 's biggest company.
\end{boxedminipage}
\caption{
Comparison of output of 3 abstractive summarization models on a news article.
The baseline model makes \error{factual errors}, a \error{nonsensical sentence} and struggles with OOV words \textit{muhammadu buhari}.
The pointer-generator model is accurate but \reph{repeats} \reph{itself}.
Coverage eliminates repetition.
The final summary is composed from \fph{several fragments}.
}
\label{summarization_examples}
\end{figure}

==> figs/tasks.tex <==
\begin{table}[h]
%{\renewcommand{\arraystretch}{1.25}
%\setlength{\tabcolsep}{12pt}
\begin{tabular}{l c}
Task & Input \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2}
Summarization & Natural Language \\ 
Translation & Multilingual \\
\cmidrule(lr){1-2}
Question Generation & Structured \\ 
\cmidrule(lr){1-2}
Image Captioning & Multimodal \\ 

\bottomrule
\end{tabular}
\caption{To validate our method, we evaluate on a diverse set of conditional natural language generation tasks}
\label{table:tasks}
\end{table}

==> figs/translation_bad.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l c c c c c}
\toprule

Model & IWSLT14 de-en \\

%\cmidrule(r){1-1}

\midrule
RNMT (6 layer) & $23.2$ \\
Coverage & $RUNNING$ \\
Transformer (6 layer)& $25.4$ \\
Scratchpad (3 layer)& $\mathbf{28.08}$ \\
% for epochs, - is inclusive, so 1-4 includes epoch 4::
%initial 3layer train, avg last 5 epochs + beam=4 -> 26.79
%initial 3layer train, avg last 5 epochs + beam=8 -> 27.05
%new 3layer train (initial + label smooth), avg epochs 11, 12, 13 +beam=8 -> 27.77
%new 3layer train (initial + label smooth), avg epochs 11-15 +beam=8 -> 27.95
%new 3layer train (initial + label smooth), stop when lr < 0.0002 (epoch20). avg last 10 epochs. +beam=12 -> 28.03
%new 3layer train (initial +label smooth), stop when lr < 0.0008 (epoch 15). avg last 5 epochs. +beam=16 -> 28.08

\bottomrule
\end{tabular}
\caption{Translation}
\label{table:translation}
\end{table*}
%Seq2Seq with Attention (6 layer) & $27.61$\\
%Coverage & $RUNNING$ \\
%Transformer (6 layer)& $32.30$ \\
%Scratchpad (3 layer)& $\mathbf{33.83}$ \\

%\begin{enumerate}
%    \item \textit{\textbf{Updates}} its state ($\s^i$) using the last output token ($y^{i-1}$) and the attentive read from the previous step ($\attn^{i-1}_\textit{read}$)
%    \item \textit{\textbf{Reads}} attentively ($\aread$) from the encoder outputs ($\enchs$) using the new state ($\s^{i+1}$) to use in the next timestep $i+1$.
%    \end{enumerate}


==> figs/translation_hyperparams.tex <==
\begin{table}[H]
\centering
%\begin{adjustbox}{width={\columnwidth}}
\begin{tabular}{l c}
\toprule
Hyperparam & Value \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2}
bpe size & $10000$ \\
word embed dim & $128$ \\
dropout (enc+dec) & $0.1$ \\

\bottomrule
\end{tabular}
\label{table:translation_hyperparams}
%\end{adjustbox}
\end{table}
